A unified decision making framework for supply and demand management in microgrid networks

This paper considers two important problems -- on the supply-side and demand-side respectively and studies both in a unified framework. On the supply side, we study the problem of energy sharing among microgrids with the goal of maximizing profit obtained from selling power while at the same time not deviating much from the customer demand. On the other hand, under shortage of power, this problem becomes one of deciding the amount of power to be bought with dynamically varying prices. On the demand side, we consider the problem of optimally scheduling the time-adjustable demand - i.e., of loads with flexible time windows in which they can be scheduled. While previous works have treated these two problems in isolation, we combine these problems together and provide a unified Markov decision process (MDP) framework for these problems. We then apply the Q-learning algorithm, a popular model-free reinforcement learning technique, to obtain the optimal policy. Through simulations, we show that the policy obtained by solving our MDP model provides more profit to the microgrids.

==> flowchart.tex <==
\tikzstyle{decision} = [diamond, draw, fill=gray!30, 
    text width=4.5em, text badly centered, node distance=3cm, inner sep=0pt]
\tikzstyle{block} = [rectangle, draw, fill=blue!20, 
    text width=6em, text centered, rounded corners, minimum height=4em]
\tikzstyle{line} = [draw, -latex']
\tikzstyle{cloud} = [draw, ellipse,fill=red!20, node distance=3cm,
    minimum height=2em]
    
\begin{tikzpicture}[node distance = 2.5cm, auto]
    % Place nodes
   \node [block] (RL) {RL Agent};
    \node [block, below of = RL] (state) {Gets state information as in };
    \node [block, below of = state] (action) {Picks actions $u_{t}$ and $v_{t}$};
    \node[block, below of = action] (ADL) { using $v_{t}$, meet the ADL-demand};
    \node[block, below of = ADL] (pass) {Pass the un-met feasible ADL jobs to the next time period};
     
    
    \node [decision, right of = ADL] (dec) {If $u_{t} + v_{t} \geq 0$};
    \node [block, right of = dec] (sell) {Sell the power to neighboring microgrids};
  %  \node [block, right of = sell] (exit1) {Exit};
    
    \node[decision, below of = dec] (newdec){If $u_{t} \leq 0$};
    \node [block, below of = newdec] (exit) {Exit};
    \node[block, right of = newdec] (non-adl) {Meet the Non-ADL demand};
    \node[decision, below of = non-adl] (batterydec) {If $nd_{t}-u_{t} \geq 0$ };
%    \node[block, right of = batterydec] (fill) {Fill the remaining in the battery};
    
   % \node [block, below of = action] (non-ADL) {using $u_{t}$, meet the non-ADL demand};
    
    %\node[decision, below of = non-ADL] (   )
    %\node [cloud, left of=init] (expert) {expert};
    %\node [cloud, right of=init] (system) {system};
    %\node [block, below of= RL] (pick) {Pick $u_{t}$};
    %\node [block, below of= pick] () {evaluate candidate models};
    %\node [block, left of=evaluate, node distance=3cm] (update) {update model};
   % \node [decision, below of=evaluate] (decide) {is best candidate better?};
    %\node [block, below of=decide, node distance=3cm] (stop) {stop};
    % Draw edges
   \path [line] (RL) -- (state);
    \path [line] (state) -- (action);
    \path [line] (action) -- (ADL);
   \path [line] (ADL) -- (pass);
   \path [line] (pass) |- (exit);
  \path [line] (action) -| (dec);
  \path [line] (dec) --  node {Yes} (sell);
 % \path [line] (sell) -- (exit1);
  \path [line] (dec) --  node {No} (newdec);
  \path [line] (newdec) --  node {No} (exit);
  \path [line] (newdec) -- node {Yes} (non-adl);
  \path [line] (non-adl) -- (batterydec);
 % \path[line] (batterydec) -- node {Yes} (fill);
  \path [line] (batterydec) -- node {No} (exit);
  %\path [line] (fill) -- (exit1);
   
  %  \path [line] (update) |- (identify);
  %  \path [line] (decide) -- node {no}(stop);
    %\path [line,dashed] (expert) -- (init);
    %\path [line,dashed] (system) -- (init);
    %\path [line,dashed] (system) |- (evaluate);
\end{tikzpicture}

